Explainable Recommender with Geometric Information Bottleneck

Explainable recommender systems can explain their recommendation decisions, enhancing user trust in the systems. Most explainable recommender systems either rely on human-annotated rationales to train models for explanation generation or leverage the attention mechanism to extract important text spans from reviews as explanations. The extracted rationales are often confined to an individual review and may fail to identify the implicit features beyond the review text. To avoid the expensive human annotation process and to generate explanations beyond individual reviews, we propose to incorporate a geometric prior learnt from user-item interactions into a variational network which infers latent factors from user-item reviews. The latent factors from an individual user-item pair can be used for both recommendation and explanation generation, which naturally inherit the global characteristics encoded in the prior knowledge. Experimental results on three e-commerce datasets show that our model significantly improves the interpretability of a variational recommender using the Wasserstein distance while achieving performance comparable to existing content-based recommender systems in terms of recommendation behaviours.

==> sections/bio.tex <==
\section{Biography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{iclr2023/bio/HanqiYan.jpg}}]{Hanqi Yan} is a third-year PhD student at the University of Warwick, UK, and a visiting PhD student at King's College London. Her research interest is Natural Language Processing, focusing on interpretable and robust NLP models. She has published several papers in top conferences and high-impact journals. Hanqi obtained her MSc and BEng degrees from Peking University, China and Beihang University, China, respectively.
\end{IEEEbiography}
\vspace{-10pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/lingui.jpg}}]{Lin Gui} is a Lecturer at the Department of Informatics, King's College London. His research interests include natural language processing, machine learning, text and data mining, sentiment analysis, and social media analysis. Lin obtained his PhD and MEng degrees in computer science from Harbin Institute of Technology, and his BASc degree in Mathematics from Nankai University, China.
\end{IEEEbiography}
\vspace{-10pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{iclr2023/bio/menghanwang.png}}]{Menghan Wang} is an Applied Researcher at eBay inc., working on developing and deploying scalable and extensible recommendation algorithms. Previously, I worked as a senior algorithm engineer in the search and recommendation team at Alibaba inc., where I developed web-scale search $\&$ recommendation algorithms and published several papers in top-tier conferences. In 2019, I obtained my PH.D. in Computer Science at Zhejiang University.
\end{IEEEbiography}
\vfill
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{iclr2023/bio/KunZhang_SmallSquare.png}}]{
Kun Zhang} is an Associate Professor with the Department of Philosophy and an Affiliate Faculty Member with the Machine Learning Department, Carnegie Mellon University, Pittsburgh, PA, USA, and an associate professor of Machine Learning at Mohamed bin Zayed University of Artificial Intelligence. His research interests lie in causality, machine learning, and artificial intelligence, especially in causal discovery, hidden causal representation learning, transfer learning, and general-purpose artificial intelligence. Dr. Zhang is a general $\&$ program co-chair for the 2022 Conference on Causal Learning and Reasoning (CLeaR), a program co-chair of the UAI 2022, % Conference on Uncertainty in Artificial Intelligence (UAI), 
and a general co-chair of the UAI 2023. %2022 Conference on Uncertainty in Artificial Intelligence (UAI).
\end{IEEEbiography}
 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/YulanHe.jpg}}]{Yulan He} is a Professor in Natural Language Processing (NLP) at King's College London and an Honorary Professor at the University of Warwick, UK. Her research centers on the integration of machine learning and NLP for text understanding. She currently holds a five-year Turing AI Fellowship, funded by the UK Research and Innovation. She has received several prizes and awards, including a SWSA Ten-Year Award, a CIKM 2020 Test-of-Time Award, and AI 2020 Most Influential Scholar (Honourable Mention) by AMiner. She has served as a Program Co-Chair for EMNLP 2020 and the General Chair for AACL-IJCNLP 2022. Yulan obtained her PhD degree in Spoken Language Understanding from the University of Cambridge. 
\end{IEEEbiography}

